Improving Deep Policy Gradients with Value Function Search

Deep Policy Gradient (PG) algorithms employ value networks to drive the learning of parameterized policies and reduce the variance of the gradient estimates. However, value function approximation gets stuck in local optima and struggles to fit the actual return, limiting the variance reduction efficacy and leading policies to sub-optimal performance. This paper focuses on improving value approximation and analyzing the effects on Deep PG primitives such as value prediction, variance reduction, and correlation of gradient estimates with the true gradient. To this end, we introduce a Value Function Search that employs a population of perturbed value networks to search for a better approximation. Our framework does not require additional environment interactions, gradient computations, or ensembles, providing a computationally inexpensive approach to enhance the supervised learning task on which value networks train. Crucially, we show that improving Deep PG primitives results in improved sample efficiency and policies with higher returns using common continuous control benchmark domains.

==> Sections/additional_statements.tex <==
\section{Ethics Statement}

The proposed Value Function Search does not focus on experiments involving human subjects and does not require sensitive data that involve sex, gender, and diversity analysis. Hence, we do not consider the gender dimension, privacy, data governance issues, or any primary ethic concern highlighted in the \textit{ICLR Code of Ethics}\footnote{https://iclr.cc/public/CodeOfEthics} to be relevant.

However, according to the \textit{"Ethics Guidelines for Trustworthy Artificial Intelligence"} report published by the High-Level Expert Group on AI of the European Commission,\footnote{https://digital-strategy.ec.europa.eu/en/library/ethics-guidelines-trustworthy-ai} ethical consideration has to take into account the environment and the sustainability of AI systems.
Regarding the environmental impact, it is crucial to foster sample efficiency (i.e., reducing the training time for the agents, hence the computational resources used to train them) of Deep RL to lower energy consumption and related emissions. In this direction, VFS leads to significant benefits in sample efficiency, which reduces the environmental footprint of VFS-based approaches by a considerable margin.

In more detail, we employed the Machine Learning CO2 impact calculator \citep{CO2} to estimate the CO2 emissions of our experiments.\footnote{We note that this is not a precise measurement as it is not trivial to map energy consumption to CO2 emissions (i.e., the carbon footprint). To this end, we employed open-source electricity maps (e.g., https://www.electricitymaps.com) to estimate better how carbon-intensive our experiment's electricity is.} According to our hardware, the carbon efficiency of the provider, and the length of our experiments, we computed a total emission of $\approx 52.3$ kg CO2. We plan to cope with such emissions using Treedom\footnote{https://www.treedom.net}, an online service that allows us to plant trees to cope with our carbon footprint. 

\section{Reproducibility Statement}
Significant efforts have been made to ensure the reproducibility of VFS. Section 3 detail the flow of VFS-based algorithms with pseudocode and detailed explanations. We also highlight possible limitations of our approach in Section 3.1. Moreover, Section 4 states our experimental setup, while supplemental material contains a detailed overview of the considered hyperparameters. 
